Graph2Plan: Learning Floorplan Generation from Layout Graphs

We introduce a learning framework for automated floorplan generation which combines generative modeling using deep neural networks and user-in-the-loop designs to enable human users to provide sparse design constraints. Such constraints are represented by a layout graph. The core component of our learning framework is a deep neural network, Graph2Plan, which converts a layout graph, along with a building boundary, into a floorplan that fulfills both the layout and boundary constraints. Given an input building boundary, we allow a user to specify room counts and other layout constraints, which are used to retrieve a set of floorplans, with their associated layout graphs, from a database. For each retrieved layout graph, along with the input boundary, Graph2Plan first generates a corresponding raster floorplan image, and then a refined set of boxes representing the rooms. Graph2Plan is trained on RPLAN, a large-scale dataset consisting of 80K annotated floorplans. The network is mainly based on convolutional processing over both the layout graph, via a graph neural network (GNN), and the input building boundary, as well as the raster floorplan images, via conventional image convolution.

==> figures/complex.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/complex.pdf}
\caption{\rh{Floorplans generated for input boundaries with the same shape but different front door locations.}}
\label{fig:complex}
\end{figure}


==> figures/gt_box.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/gt_box.png}
\caption{
\rh{Generation of ground-truth bounding boxes of rooms. (a) Given the boxes obtained after removing the floorplan walls, (b) we align the boxes to the building boundary, and then (c) align adjacent boxes to each other.
%ground-truth room box alignment
} }
\label{fig:gt_box}
\end{figure}

